Evaluating 3D User Interaction Techniques on Spatial Working Memory for 3D Scatter Plot Exploration in Immersive Analytics

This work evaluates three 3D user interaction techniques to investigate their visuo-spatial working memory support for users' data exploration in immersive analytics. Two techniques are the common VR locomotion technique, Walking and Teleportation, while the other one is Grab, an object manipulation technique. We present two formal user studies in VR and AR. Our study is designed based on the Corsi block-tapping Task, a psychological test for assessing visuo-spatial working memory. Our study results show that Walking supports spatial memory best, and Grab follows. Though Teleportation is found to support it the least, participants rated Teleportation as the easiest way to move in the VR study. We also compare the Walking and Grab results in the VR and AR studies and discuss differences. At last, we discuss our limitations and future work.

==> Contents/6_vr_vs_ar__old_.tex <==
\section{Comparison between VR and AR}

% In the earlier sections, we reported the results of our studies in VR and AR. 
In the earlier sections, we reported the results of the VR and AR studies. 
% This section compares the outcomes for VR and AR environments. 
This section compares these outcomes. 
The mixed-designed ANOVA test is used to compare the VR and AR results by the interaction techniques and view transition angles at the 5\% significance level. The environments of VR and AR serve as the between-subject factor, and the interaction techniques and degrees of view transition serve as the within-subject factors.
% The between-subject ANOVA test is used to analyze and report the results for VR and AR at the 5\% significance level. 
% \ic{try mixed ANOVA, VR/AR x interaction x degree}

The distance errors and interaction time are the measurements to be analyzed. \HDY{For a tapping task, its index of difficulty (ID) is measured by calculating movement distance from an object to the target object divided by target object size according to Fitt's law~\cite{fitts1954information}. As stated in Section 3.2, both physical size of a target and the average travel distance to tap the target shrank by the same ratio of 0.6 in the AR study compared to theirs in the VR study. This means that the IDs for our VR and AR research are the same. This rationale allows us to compare the results of the two studies.} 
% \HDY{According to Fitt's law~\cite{fitts1954information}, the VR and AR studies have the same index of difficulty (ID), which is measured by calculating movement distance from an object to the target object divided by target object size. This rationale allows us to compare the results of the two studies.} 
To compare the distance error results, we perform data pre-processing. 
% Due to the field of view restriction of the AR device, each axis of the 3D scatter plot in AR is 0.6 times larger than the axis of the VR scatter plot, as we explained in Section X. 
As we explained in Section~\ref{subsection_scatterPlot}, each axis of the 3D scatter plot in AR is 0.6 times larger than the axis of the VR scatter plot.
% due to the smaller field of view of Hololens 2.
We normalize the VR distance error by multiplying 0.6. 
% We normalize the distance by dividing the VR error distances by 0.6. 
In the case of interaction times, pre-processing is not required. This is because the tasks in both environments ask a participant to move in the IE or rotate the plots so that they can view a 90\degree{} or 180\degree{} rotated view of the current view, 75 cm away from the center of the plot.
% In the case of interaction time, pre-processing is not required. This is due to the fact that the tasks in both environments ask participants to move so that they can view a 90- or 180-degree rotated view of the current view, 75 cm away from the center of the plot.
We set the following hypotheses:

\begin{enumerate}
[label=H\arabic*., noitemsep, ]
\setcounter{enumi}{7}
\item The distance errors in VR will be much smaller than in AR. We expect this because VR users could focus more on 3D plots than AR users due to their background characteristics. Real-world objects around the plots might distract AR users.

\item Walking in VR and AR will not have a difference in interaction time. This is due to the fact that Walking is dependent on users' own ability and is not characterized by technical differences.

\item Grab in VR and AR will have significantly different interaction times due to their technical differences (i.e., controller vs. pinch gesture) in interacting with the plots. 

\end{enumerate}
\vspace{-.4cm}
% \begin{table}[ht]
% \caption{\label{table_result_mixed_anova_errorDistance} \textbf{VR vs. AR: Statistical Results on Error Distance}}
% \begin{tabular}  {m{4.3cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
% \toprule
%     {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
%     \textbf{Within-Subjects}\\
%     % Tech. \texttimes View Transition Angle \texttimes IE & {1, 138} & {.914} & {.341} & {.007} \\
%     Tech. \texttimes View Transition Angle & {1, 138} & {.290} & {.591} &{.002}\\
%     View Transition Angle \texttimes IE & {1, 138} & {3.08} & {\textless.001} & {.086}\\
%     Tech.  \texttimes IE & {1, 138} & {7.87} & {.006} & {.054}\\
%     Tech. & {1, 138} & {9.13} & {.003} & {.062} \\
%     View Transition Angle & {1, 138} & {13.0} & {\textless .001} & {.086}\\\midrule
%     \textbf{Between-Subjects}\\
%     IE (VR vs. AR) & {1, 138}& 276& \textless.001 & .667\\ 
%     \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[ht]
\small
\caption{\label{table_result_mixed_anova_errorDistance} \textbf{VR vs. AR: Results on Distance Error}}
\begin{tabular}  {m{4.0cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
\toprule
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    \textbf{Within-Subjects}\\
    % Tech. \texttimes View Transition Angle \texttimes IE & {1, 138} & {.914} & {.341} & {.007} \\
    Technique \texttimes{} View Transition Angle & {1, 138} & {.044} & {.833} &{.001}\\
    Technique  \texttimes{} Tapping Order & {2, 276} & {.009} & {.991} & {.001}\\
    View Transition Angle \texttimes{} Tapping Order & {2, 276} & {1.21} & {.299} & {.009}\\
    View Transition Angle \texttimes{} IE & {1, 138} & {.031} & {.860} & {.001}\\
    Tapping Order \texttimes{} IE & {2, 276} & {.593} & {.554} & {.004}\\
    Technique  \texttimes{} IE & {1, 138} & {2.24} & {.136} & {.016}\\
   
    
    Technique & {1, 138} & {4.393} & {.038} & {.031} \\
    View Transition Angle &{1, 138} & {10.4} & {.002} & {.070}\\
    Tapping Order & {2, 276} & {5.46} & {.005} & {.038}\\\midrule
    \textbf{Between-Subjects}\\
    IE (VR vs. AR) & {1, 138}& {11.4}& \textless.001 & .077\\ 
    \bottomrule
\end{tabular}
\vspace{-.3cm}
\end{table}

% \begin{table}[ht]
% \caption{\label{table_result} \textbf{VR vs. AR: Statistical Results on Error Distance}}
% \begin{tabular}  {m{4.3cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
% \toprule
%     {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
%     Walking * 90\textdegree  & {1, 128} & {.012}  & {.911} & {\textless .001} \\ 
%     Walking * 180\textdegree  & {1, 128} &  {.089}  & {.766} & {.001} \\
%     Steering * 90\textdegree & {1, 128}  & {1.64} & {.202} & {.013} \\
%     Steering * 180\textdegree & {1, 128}  & {11.7} & {\textless .001} & {.084} \\
%     \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[ht]
% \caption{\label{table_result} \textbf{VR vs. AR: Statistical Results on Interaction Time}}
% \begin{tabular} {m{4.3cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
% \toprule
%     {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
%     Walking * 90\textdegree  & {1, 128} & {67.1}  & {\textless.001} & {.344} \\ 
%     Walking * 180\textdegree  & {1, 128} &  {18.7}  & {\textless.001} & {.128} \\
%     Steering * 90\textdegree & {1, 128}  & {68.7} & {\textless.001} & {.349} \\
%     Steering * 180\textdegree & {1, 128}  & {32.4} & {\textless.001} & {.202} \\
%     \bottomrule
% \end{tabular}
% \end{table}

\textbf{Distance Error}
Statistical results are reported in Table~\ref{table_result_mixed_anova_errorDistance}. No interaction effects between the independent variables are found.
% except between the interaction techniques and IE types ($p$=.030).
% interaction techniques and view transition angles is reported ($p$=.591). 
% We find an interaction effect between view transition angles and IE types ($p$\textless.001). Simple effects on IE types when the view transition angle is 90- ($p$\textless .001) and 180-degrees ($p$\textless .001) are found. For the 90-degree condition, VR ($m$=.236, SD=.235) has statistically less errors than AR ($m$=.399, SD=.526). Under the 180-degree condition, similarly, VR ($m$=.295, SD=.238) has statistically less errors than AR ($m$=.568, SD=.620). 
% An interaction effect between the interaction techniques and IE types is reported ($p$=.030).
% For the further analysis on the interaction effect between the techniques and IE types, a simple effect on the IE types are found for Steering ($p$=.010). Steering ($m$=.149, SD=.174) in VR has significantly less errors than Steering ($m$=.189, SD=.271) in AR respectively. No simple effect for Walking ($p$=.448) in VR and AR is found.
Main effects of the interaction techniques ($p$=.038) and view transition angles ($p$=002) are found. Their pairwise comparison results say Walking ($m$=.073, SD=.096) has statistically smaller distance errors than Grab ($m$=.082, SD=.102), and the smaller transition movements ($m$=.068, SD=.094) have significantly lower errors than larger movements ($m$=.087, SD=.104). A main effect of the tapping orders is also reported ($p$=.005). In its pairwise comparisons, the first order of tapping has ($m$=.067, SD=.093) statistically smaller distance errors than the second ($m$=.082, SD=.101, $p$=.022) and third taps ($m$=.083, SD=.102, $p$=.022). Distance errors in the second and third taps show no difference ($p$=1.00). Regarding the IE types, we find the distance errors in AR ($m$=.058, SD=.090) are statistically less than in VR ($m$=.088, SD=.103). 
These findings reject our H8.
% These findings are opposite to our H7.

% Statistical results are reported in Table~\ref{table_result_mixed_anova_errorDistance}. First of all, we find that Walking has no effect on the error distances for the required view transition angles in VR and AR. For Steering, on the other hand, we found a significant difference between error distances in 180\textdegree{} view transition between VR and AR. Steering in VR has a smaller error distance than in AR. No significant difference for Steering in 180\textdegree{} view transition is found.


\begin{table}[ht]
\small
\caption{\label{table_result_mixed_anova_interactionTime} \textbf{VR vs. AR: Results on Interaction Time}}
\begin{tabular}  {m{4.0cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
\toprule
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    \textbf{Within-Subjects}\\
    % Tech. \texttimes View Transition Angle \texttimes IE & {1, 138} & {.028} & {.868} & {.001} \\
    Technique \texttimes View Transition Angle & {1, 138} & {.194} & {.660} &{.001}\\
    View Transition Angle \texttimes IE & {1, 138} & {1.20} & {.274} & {.009}\\
    Technique  \texttimes IE & {1, 138} & {16.2} & {\textless.001} & {.105}\\
    Technique & {1, 138} & {72.7} & {\textless.001} & {.345} \\
    View Transition Angle & {1, 138} & {41.6} & {\textless .001} & {.232}\\ \midrule
    \textbf{Between-Subjects}\\
    IE (VR vs. AR) & {1, 138}& {1783}& {\textless.001} & {.928}\\
    \bottomrule
\end{tabular}
\vspace{-.4cm}
\end{table}

\textbf{Interaction Time} We report the statistical analysis results in Table~\ref{table_result_mixed_anova_interactionTime}. 
% We found no interaction effects between the techniques, view transition angles, and IE types ($p$=.868). 
There are no interaction effects between the techniques and view transition angles ($p$=.660) and between view transition angles and IE types ($p$=.274). However, the techniques and IE types show an interaction effect ($p$\textless.001). We find simple effects on the IE types for Grab ($p$\textless.001) and Walking ($p$\textless.001). In their pairwise comparisons, Grab ($m$=8.91, SD=4.59) and Walking ($m$=7.41, SD=3.09) in VR are significantly faster interaction times than Grab ($m$=14.6, SD=6.05) and Walking ($m$=10.4, SD=3.18) in AR. These findings support H10 but reject H9.

Main effects of the interaction techniques ($p$\textless.001) and view transition angles ($p$\textless.001) are found. A pairwise comparison result indicates Walking ($m$=8.49, SD=3.44) has a statistically faster interaction time than Grab ($m$=10.9, SD=5.83). In addition, the smaller transition movements ($m$=8.69, SD=4.34) have less interaction time than larger movements ($m$=10.8, SD=5.29). Regarding the IE types, we also find the interaction times in VR ($m$=8.16, SD=3.98) are statistically faster than in AR ($m$=12.5, SD=5.26).



% \begin{table}[ht]
% \small
% \caption{\label{table_result_mixed_anova_tappingCompletionTime} \textbf{VR vs. AR: Results on Tapping Completion Time}}
% \begin{tabular}  {m{4.3cm} | m{0.8cm} | m{0.5cm}| m{0.6cm} | m{0.5cm}}
% \toprule
%     {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
%     \textbf{Within-Subjects}\\
%     % Tech. \texttimes View Transition Angle \texttimes IE & {1, 138} & {.028} & {.868} & {.001} \\
%     Technique \texttimes View Transition Angle & {1, 138} & {.026} & {.872} &{.001}\\
%     View Transition Angle \texttimes IE & {1, 138} & {1.00} & {.319} & {.007}\\
%     Technique  \texttimes IE & {1, 138} & {2.81} & {.096} & {.20}\\
%     Technique & {1, 138} & {12.1} & {\textless.001} & {.080} \\
%     View Transition Angle & {1, 138} & {13.1} & {\textless .001} & {.087}\\ \midrule
%     \textbf{Between-Subjects}\\
%     IE (VR vs. AR) & {1, 138}& {96.9}& {\textless.001} & {.413}\\
%     \bottomrule
% \end{tabular}
% \vspace{-.4cm}
% \end{table}

% \paragraph{Tapping Completion Time}

% The statistical analysis results are reported in Table~\ref{table_result_mixed_anova_tappingCompletionTime}. 
% We found significant main effects, but no interaction effects. A main effect of the interaction techniques ($p$\textless.001) is found. Its pairwise comparison indicates Walking ($m$=30.5s, SD=14.1) has a statistically faster tapping completion time than Steering ($m$=33.9s, SD=15.8). In addition, a main effect of the view transition angles ($p$\textless.001) is found. The smaller transition movements ($m$=30.6s, SD=13.6) have less completion time than larger movements ($m$=33.8s, SD=16.3). For the IE types, at last, the participants in VR ($m$=24.7s, SD=8.78) complete the tasks much faster than the other participants in AR ($m$=40.0s, SD=18.5).


==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

